Graph-based Detection of Multiuser Impulse Radio Systems

Impulse-Radio (IR) is a wideband modulation technique that can support multiple users by employing random Time-Hopping (TH) combined with repeated transmissions. The latter is aimed at alleviating the impact of collisions. This work employs a graphical model for describing the multiuser system which, in turn, facilitates the inclusion of general coding schemes. Based on factor graph representation of the system, several iterative multiuser detectors are presented. These detectors are applicable for any binary linear coding scheme. The performance of the proposed multiuser detectors is evaluated via simulations revealing large gains with low complexity.

==> FP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{FP detector}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\label{sec:FP_decoder}
%
%For completeness, % of the presentation,
%We briefly review the FP decoder \cite{fishler-lowcomplexity} for
%completeness and since the definitions and terminology . This
%decoder will not be analyzed herein and the reader can skip this
%section to \ref{sec:ID_decoder}.
The FP detector
%was tailored for a
%system employing a repetition code. The decoder
consists of two stages performed in an iterative manner.
%
In the first stage, termed {\it pulse detection}, the \emph{a
posteriori} log likelihood ratio (LLR) is calculated given the
received signal and the information transmitted by other colliding
users.
%
In the second stage, {\it symbol detection}, the \emph{a
posteriori} LLR is calculated given the information from the pulse
detector. % of the corresponding user.
The symbol detector uses the fact that all the pulses of the
\emph{k}th user correspond to the same bit.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsubsection{First stage - pulse detection}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

In the pulse detection stage, the \emph{a posteriori}
log-likelihood ratio (LLR) of $b^k_j$ is calculated using
\begin{equation}\label{fp-ex1}
\begin{split}
    L_1(b^k_j) &= log\frac{Pr\left( b^k_j = 1 | r \right) }{ Pr\left( b^k_j = -1 | r \right)}\\
               &= log\frac{ f \left( r | b^k_j=1 \right) }{ f \left( r | b^k_j=-1 \right) } +
                        log\frac{Pr\left( b^k_j = 1 \right) }{ Pr\left( b^k_j = -1
                        \right)},
\end{split}
\end{equation}
%
where $b^k_1=\ldots=b^k_{N_f}$ are symbols transmitted by the
\textit{k}th user via $N_f$ pulses. It can be shown that the first
term of \eqref{fp-ex1} is
%
\begin{equation}\label{fp-ex2}
\begin{split}
        %&log\frac{Pr\left( b^k_j = 1 \right) }{ Pr\left( b^k_j = -1 \right)} = \\
                &log\frac{ f \left( r | b^k_j=1 \right) }{ f \left( r | b^k_j=-1 \right) } = \\
        &log\frac{ \sum_{b\in\left\{ \pm1 \right\}^{K^j_k}}
                           e^{-\frac{\left(r_{l(j,m)}-\overline{1}\cdot A^j_k[1, b]^T\right)^2}{2\sigma_n^2} }
                           p\left( b \right)}
                        { \sum_{b\in\left\{ \pm1 \right\}^{K^j_k}}
                           e^{-\frac{\left(r_{l(j,m)}-\overline{1}\cdot A^j_k[-1, b]^T\right)^2}{2\sigma_n^2} }
                           p\left( b \right)}
        \equiv \lambda_1^j \left( b_i^k \right),
\end{split}
\end{equation}
%
where $\overline{1}$ denotes the all-one vector, $A^j_k$ is a
diagonal matrix containing the amplitudes of the pulses received
from the $k$th user and the users colliding with the \emph{j}th
pulse of the $k$th user, $K^j_k$ is the number of such collisions.
%users colliding with the \emph{j}th pulse of the
%\emph{k}th user.
$p\left(b\right)$ can be calculated from the extrinsic information
obtained from the second stage (i.e. from the previous iteration
of the symbol detector). $\lambda_1^j \left( b_i^k \right)$ is the
extrinsic information that is fed to the second stage.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsubsection{Second stage - symbol detection}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

In the symbol-detection stage, the \emph{a posteriori} LLR of the
transmitted information symbol is calculated given the \emph{a
priori} LLR values from the pulse detector stage.
%
% OFER: xxx why is the index "n" introduced here ? can we replace "n" with "j", and "j" with "i" to
% be consistent with Eq. (18) ? (17) ? it is very easy to get lost here .
\begin{equation}\label{fp-ex3}
\begin{split}
    &L_2^n(b_j^k)  \\
                            &=log\frac{Pr\left( b^k_j = 1 | \lambda_1^n \left( b_j^m \right), j=1,\ldots,N_f , m=1,\ldots,K \right)  }
                    {Pr\left( b^k_j = -1 | \lambda_1^n \left( b_j^m \right), j=1,\ldots,N_f , m=1,\ldots,K \right)  }\\
                &=log\frac{Pr\left( b^k_j = 1 | \lambda_1^n \left( b_j^k \right), j=1,\ldots,N_f\right)  }
                    {Pr\left( b^k_j = -1 | \lambda_1^n \left( b_j^k \right), j=1,\ldots,N_f\right)
                    }.
\end{split}
\end{equation}

It can be shown that
\begin{equation}\label{fp-ex4}
\begin{split}
    L_2^n\left(b_j^k\right)
%                                                &= \sum_{l=1}^{N_f}log
%                                                     \frac{Pr\left( b^k_l =  1 | \lambda_1^n \left( b_l^k \right) \right) }
%                                   {Pr\left( b^k_l = -1 | \lambda_1^n \left( b_l^k \right) \right) } \\
%                           &= \sum_{l=1,l\neq{j}}^{N_f}log
%                                   \frac{Pr\left( b^k_l =  1 | \lambda_1^n \left( b_l^k \right) \right) }
%                                   {Pr\left( b^k_l = -1 | \lambda_1^n \left( b_l^k \right) \right) } \\
%                           & +\frac{Pr\left( b^k_j =  1 | \lambda_1^n \left( b_j^k \right) \right) }
%                                   {Pr\left( b^k_j = -1 | \lambda_1^n \left( b_j^k \right) \right) } \\
                           &= \underbrace{\sum_{l=1,l\neq{j}}^{N_f}
                                \lambda_1^n \left( b_l^k \right)}_{\lambda_2^n \left( b_j^k \right)}
                              + \lambda_1^n \left( b_j^k\right).
\end{split}
\end{equation}
%
The output of the symbol stage is the sum of inputs from the pulse
detector.
%

The graph that we associate with the FP detector is a bipartite graph.
Associated with the first stage of the decoding is the left-hand side of the graph consisting of at most $N_f N_c$ nodes,
one for each of the outputs of the matched filter $r$. We shall hence refere to these nodes as \emph{input nodes}.
%
The right hand side of the graph is associated with the second stage of the decoding. It consists of $K$ nodes, referred to as \emph{check nodes}, one for each of the $K$ users.
The connection between the two sets of nodes is determined by the matrix $S$ -
\emph{input node} $i$ is connected to \emph{check node} $j$, if
$S_{ij}=1$.

Returning to the toy example of Figure~\ref{fig:SystemModel}, the
corresponding $S$ matrix is given by
%
\begin{equation}\label{s_for_example}
\mathbf{S^T}= \left[
\begin{array}{ccccc ccccc ccccc}
0 & 1 & 0 & 0 & 0     & 1 & 0 & 0 & 0 & 0     & 0 & 0 & 0 & 1 & 0  \\
0 & 0 & 1 & 0 & 0     & 1 & 0 & 0 & 0 & 0     & 1 & 0 & 0 & 0 & 0  \\
\end{array} \right],
\end{equation}
%
and Figure~\ref{fig:simple_iterative_graph} presents
the %factor %% OFER: I removed "factor" since this is defined later on!
graph we associate with the FP detector.
%
\begin{figure}[ht]
    \centering
    \includegraphics[width=200pt]{eps/simple_iterative}
    \vspace*{-1.5cm}
    \caption{FP decoder graph: $K=2$ users, $N_f=3$ frames, $N_c=5$ chips per frame.}
    \label{fig:simple_iterative_graph}
\end{figure}
\vspace*{-1.2cm}


==> macros.tex <==
%%%%%%%%%%%  Page length parameters %%%%%%%%%%%%%
% Dense format
\def\denseformat{
\setlength{\textheight}{9in}
\setlength{\textwidth}{6.9in}
\setlength{\evensidemargin}{-0.2in}
\setlength{\oddsidemargin}{-0.2in}
\setlength{\headsep}{10pt}
\setlength{\topmargin}{-0.3in}
\setlength{\columnsep}{0.375in}
\setlength{\itemsep}{0pt}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mid format
\def\midformat{
\setlength{\textheight}{8.9in}
\setlength{\textwidth}{6.7in}
\setlength{\evensidemargin}{-0.2in}
\setlength{\oddsidemargin}{-0.2in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}       % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.1}
\parskip=0.070in
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spacy format
\def\spacyformat{
\setlength{\textheight}{8.8in}
\setlength{\textwidth}{6.7in}
\setlength{\evensidemargin}{-0.18in}
\setlength{\oddsidemargin}{-0.18in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}      % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.2}
\parskip=0.080in
}

\def\tauformat{ %A4 only
\setlength{\textheight}{9.2in}
\setlength{\textwidth}{6.7in}
\setlength{\evensidemargin}{-0.2in}
\setlength{\oddsidemargin}{-0.2in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}       
\setlength{\footskip}{.8in}
\renewcommand{\baselinestretch}{1.1}
\parskip=0.070in
}


%%%%%%%%%%%%  Defining theorem-like environments %%%%%%%%%%
\ifx\thmsection\undefined
\def\thmsection{section}
\fi

\newtheorem{theorem}{Theorem}[\thmsection]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}{Definition}[\thmsection]
\newtheorem{algorithm}{Algorithm}[\thmsection]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}{Conjecture}
\newtheorem{notation}[definition]{Notation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}{Observation}
%\newtheorem{comment}{Comment}
\newtheorem{assumption}{Assumption}[\thmsection]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\weizprinter{\setlength{\topmargin}{0.3in}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\boldhead#1:{\par\vskip 7pt\noindent{\bf #1:}\hskip 10pt}
\def\ithead#1:{\par\vskip 7pt\noindent{\it #1:}\hskip 10pt}
\def\inline#1:{\par\vskip 7pt\noindent{\bf #1:}\hskip 10pt}
%
%The next command is essentially equivalent to \section*,
%except smaller font
\def\heading#1{\par\medskip\noindent{\bf #1}\par\smallskip\noindent}
\long\def\comment #1\commentend{}
\long\def\commfull #1\commend{#1}
\long\def\commabs #1\commenda{}
\long\def\commtim #1\commendt{#1}
\long\def\commb #1\commbend{}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def\QED{\quad\blackslug\lower 8.5pt\null\par}
\def\Qed{\QED}
\def\inQED{~~~~~\quad\blackslug\lower 8.5pt\null}
\def\Proof{\noindent{\bf Proof:~}}
\def\ProofOf#1#2{\noindent{\bf Proof of #1 \ref{#2}:~}}
\def\proof{\Proof}
\def\Sketch{\noindent{\bf Proof Sketch}: }
\def\Method{\noindent{\bf Proof Method}: }
\long\def\PPP#1{\noindent{\bf Proof:}{ #1}{\quad\blackslug\lower 8.5pt\null}}
\long\def\PP#1{\noindent {\bf Proof}:{ #1} $\Box$ \\}
\long\def\P#1{{\Proof}{#1}\Qed\\}
\def\Remark{\noindent{\bf Remark:~}}
%\def\Comment{\noindent{\bf Comment:~}}
\long\def\denspar #1\densend
{#1}
%{{\renewcommand{\baselinestretch}{0.8}\small #1\par\medskip}}
\def\DEF{\stackrel{\rm def}{=}}
\newcommand{\Eqr}[1]{Eq.~(\ref{#1})}
\newcommand{\diff}{\ne}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\OO}[1]{O\left( #1\right)}
\newcommand{\OM}[1]{\Omega\left( #1 \right)}
\newcommand{\Set}[1]{\left\{ #1 \right\}}
\newcommand{\Seq}[1]{\left\langle #1 \right\rangle}
\newcommand{\Range}[1]{\left\{1,\ldots, #1 \right\}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ignore}[1]{}
\newcommand{\Exp}[1]{\mathbf{E}\left[#1\right]}
\newcommand{\Var}[1]{\mathbf{Var}\left[#1\right]}
\newcommand{\Prob}[1]{\Pr\left[ #1 \right]}
\newcommand{\EXP}[1]{\exp\Paren{#1}}


\newcommand{\inclaim}[2]{\trivlist \item[\hskip \labelsep{\bf Claim #1.}{\em #2}]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
%%%%%%%%%%%%%%%%%%
\def\hA{{\hat A}}
\def\hB{{\hat B}}
\def\hC{{\hat C}}
\def\hD{{\hat D}}
\def\hE{{\hat E}}
\def\hF{{\hat F}}
\def\hG{{\hat G}}
\def\hH{{\hat H}}
\def\hI{{\hat I}}
\def\hJ{{\hat J}}
\def\hK{{\hat K}}
\def\hL{{\hat L}}
\def\hP{{\hat P}}
\def\hQ{{\hat Q}}
\def\hR{{\hat R}}
\def\hS{{\hat S}}
\def\hT{{\hat T}}
\def\hW{{\hat W}}
\def\hX{{\hat X}}
\def\hY{{\hat Y}}
\def\hZ{{\hat Z}}
%%%%%%%%%%%%%%%%%
\def\eps{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Marginal notes for communicating with coauthors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\marginparwidth}{1in}
\setlength{\marginparpush}{-5ex}
\newif\ifnotesw\noteswtrue% T to show box & marginal notes; F supresses.
\newenvironment{change}%
   {\ifnotesw\marginpar[\hfill\(\top\)]{\(\top\)}\fi}%
   {\ifnotesw\marginpar[\hfill\(\bot\)]{\(\bot\)}\fi}
\newcommand{\deletion}{\ifnotesw\marginpar[\hfill\(\vartheta\)]{\
(\vartheta\)}\fi}
\newcommand{\mnote}[1]%
    {\ifnotesw\marginpar%
        [{\scriptsize\begin{minipage}[t]{\marginparwidth}
        \raggedleft#1%
                        \end{minipage}}]%
        {\scriptsize\begin{minipage}[t]{\marginparwidth}
        \raggedright#1%
                        \end{minipage}}%
    \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newenvironment{denselist}{
\begin{list}{(\arabic{enumi})}{
\usecounter{enumi}
\setlength{\topsep}{0pt}
\setlength{\partopsep}{0pt}
\setlength{\itemsep}{0pt}
}}{\end{list}}

\newenvironment{denseitemize}{
\begin{list}{$\bullet$}{
\setlength{\topsep}{0pt}
\setlength{\partopsep}{0pt}
\setlength{\itemsep}{0pt}
}}{\end{list}}

\newenvironment{subdenselist}{
\begin{list}{(\arabic{enumi}\alph{enumii})}{
\usecounter{enumii}
\setlength{\topsep}{0pt}
\setlength{\partopsep}{0pt}
\setlength{\itemsep}{0pt}
}}{\end{list}}

\newenvironment{namedlist}[1]{\par\vspace{1mm}\underline{#1}\vspace*{-5mm}\\
\begin{list}{(\arabic{enumi})}{
\usecounter{enumi}
\setlength{\topsep}{0pt}
\setlength{\partopsep}{0pt}
\setlength{\itemsep}{0pt}
}}{\end{list}\vspace{1mm}}





\newcommand{\handoutformat}{
        \addtolength{\topmargin}{-1.2in}
        \setlength{\oddsidemargin}{-.1 in}
        \setlength{\textwidth}{6.4in}
        \setlength{\textheight}{9.6in}
}
\newcommand{\talkformat}{
        \addtolength{\topmargin}{-1in}
        \setlength{\oddsidemargin}{-.1 in}
        \setlength{\textwidth}{6.5in}
        \setlength{\textheight}{9in}
        \parindent=0.0in
}
\def\lectureformat{
\setlength{\textheight}{8.8in}
\setlength{\textwidth}{6.5in}
\setlength{\evensidemargin}{-0.18in}
\setlength{\oddsidemargin}{-0.18in}
\setlength{\headheight}{0in}
\setlength{\headsep}{10pt}
\setlength{\topsep}{0in}
\setlength{\topmargin}{0.0in}
\setlength{\itemsep}{0in}      % 10pt is too big with the 1.2 stretch
\renewcommand{\baselinestretch}{1.2}
%\parskip=0.0in
%\parindent=0.0in
}

%\newcommand{\headersmall}[3]{
%   \pagestyle{plain}
%   \noindent
%      \vbox{
%    \hbox to 6.28in { \Course \hfill #2} 
%\hrule
%
%\vspace{1mm}
%
%Prof. Patt-Shamir
%
%       \vspace{7mm}
%
%       \hbox to 6.28in {\Large\bf \hfill #3 \hfill} 
%      }
%   \vspace*{8mm}
%}

%\newcommand{\tauheadersmall}[4]{%#1=course, #2=instructor, #3=date, #4=header
%   \pagestyle{plain}
%   \noindent
%      \vbox{
%   \vspace{-.5in}
%    \hbox to 6.28in {#1 \hfill #3}
%\hrule
%
%\vspace{1mm}
%#2\hfill
%       \vspace{7mm}
%       \hbox to 6.28in {\Large\bf \hfill #4 \hfill}
%      }
%%   \vspace*{8mm}
%   \vspace*{-6mm}
%}

%\newcommand{\lectureheader}[3]{
%   \pagestyle{plain}
%   \noindent
%      \vbox{
%    \hbox to 6.28in { \Course
%                        \hfill #2 } 
%\hrule
%\vspace*{1mm}
%Lecturer: #3
%       \vspace{7mm}\\
%       \hbox to 6.28in {\LARGE\bf \hfill Lecture #1 \hfill} 
%        }
%   \vspace*{4mm}
%}
%
%\newcommand{\newlectureheader}[3]{
%   \pagestyle{plain}
%   \noindent
%      \vbox{
%    \hbox to 6.28in { 6.04s Design and Analysis of Distributed Protocols
%                       \hfill #2} 
%\hrule
%\vspace*{1mm}
%Lecturer: #3
%       \vspace{7mm}\\
%       \hbox to 6.28in {\LARGE\bf \hfill Lecture #1 \hfill} 
%        }
%   \vspace*{4mm}
%}
%
%
%\newcommand{\talkheader}[3]{
%   \pagestyle{plain}
%   \vbox{
%    \hbox to 6.28in {Lecturer: #3 \hfill #2 } 
%    \hrule
%    \vspace*{7mm}
%    \hbox to 6.28in {\LARGE\bf \hfill #1 \hfill} 
%   }
%   \vspace*{4mm}
%}

\def\hd{\hat{\delta}}
\def\hp{\hat{p}}
\def\Lr{\Leftrightarrow}


 \def\For{{\bf for }}
 \def\To{{\bf to }}
 \def\If{{\bf if }}
 \def\Then{{\bf then }}
 \def\Else{{\bf else }}
 \def\Do{{\bf do }}
 \def\While{{\bf while }}
 \def\Continue{{\bf continue }}
 \def\Repeat{{\bf repeat }}
 \def\Until{{\bf until }}

\newcommand{\DRAFTp}{0}
\def\DRAFT{
\renewcommand{\DRAFTp}{1}
\markright{DRAFT (\today)}
\pagestyle{myheadings}
\setlength\headsep{30pt}
\setlength\topmargin{-\headsep}
}

% equations with explanations:
%\begin{eqntext}
%a & < & b & because he was born earlier
%\end{eqntext}
\newenvironment{eqntext}{\em\raggedright\[\begin{array}{rcl@{\hspace{1cm}}p{2.2in}}}{\end{array}\]}

\def\Plus{\hbox{\raise 0.3ex\hbox{\tiny +}}} % plus for international
                                             % numbers

% Responses:
% \Point{complaint, printed in tt}{response, in rm}
\newcommand{\Point}[2]{\par\bigskip\noindent$\bullet$~~\textit{\small#1}\par\noindent{#2}}



==> python_graphs/fg3_gh_simulations/fg3_gh_results.tex <==
$d_v$ & $d_c$ & Max Users & Rate & Capacity \\ \hline
3 & 4 & 56 & 0.25 & 14.00 \\
3 & 6 & 32 & 0.50 & 16.00 \\
3 & 8 & 23 & 0.63 & 14.38 \\
5 & 6 & 39 & 0.17 & 6.50 \\
5 & 8 & 28 & 0.38 & 10.50 \\
5 & 10 & 21 & 0.50 & 10.50 \\
5 & 12 & 17 & 0.58 & 9.92 \\
5 & 14 & 15 & 0.64 & 9.64 \\


==> python_graphs/simple_decoder_calc/____________________sd_method_1_results.tex <==
Dv & Dc & Max Users(1) & Max Users(2) & Rate & Capacity \\ \hline
3 & 4 & 28 & 28 & 0.25 & 7.00 \\
3 & 6 & 16 & 16 & 0.50 & 8.00 \\
3 & 8 & 12 & 12 & 0.63 & 7.50 \\
5 & 6 & 20 & 20 & 0.17 & 3.33 \\
5 & 8 & 14 & 14 & 0.38 & 5.25 \\
5 & 10 & 11 & 11 & 0.50 & 5.50 \\
5 & 12 & 9 & 9 & 0.58 & 5.25 \\
5 & 14 & 8 & 8 & 0.64 & 5.14 \\


==> python_graphs/simple_decoder_calc/sd_method_1_results.tex <==
$d_v$ & $d_c$ & Max Users(1) & Max Users(2) & Rate & Capacity \\ \hline
3 & 4 & 28 & 28 & 0.25 & 7.00 \\
3 & 6 & 16 & 16 & 0.50 & 8.00 \\
3 & 8 & 12 & 12 & 0.63 & 7.50 \\
5 & 6 & 20 & 20 & 0.17 & 3.33 \\
5 & 8 & 14 & 14 & 0.38 & 5.25 \\
5 & 10 & 11 & 11 & 0.50 & 5.50 \\
5 & 12 & 9 & 9 & 0.58 & 5.25 \\
5 & 14 & 8 & 8 & 0.64 & 5.14 \\


==> semi_multiuser.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Semi Multiuser detector for TH-IR systems}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\label{chap:smud}
% no \PARstart

%OFER: CHANGE THIS CHAPTER OPENING WORDS AFTER GOING THROUGH !!!!!

This section is dedicated for the performance analysis of the a
so-called {\it Semi} Multi-User Detector (SMUD).
%We introduce this family of detectors and obtain %calculate
%the capacity of a system employing such a detector. %SMUD.
%We will show the
%
The SMUD detects each user while treating all the others as
additive noise; since it does not consider the information
received from all users simultaneously,
%the full received information , and therefore are
it is not an optimal approach. The only multi user information
that the SMUD exploits is the knowledge of $S[i]$ (the collision
coordinates).
%, (and hence it is termed semi-MUD).

We begin by looking at the so-called %a receiver called
{\it Blinking Receiver}
%which  was
proposed by Fishler and Poor \cite{fishler-lowcomplexity}. Then,
we present a new approach for modelling the UWB-TH-IR channel
which lends itself to capacity analysis. We also discuss a coding
scheme aimed at achieving this capacity.

%It will be shown that performance improvement can be achieved by
%employing a coded scheme rather than a repetition-based scheme.
%This will also provide the motivation %and it will motivate us
%for the development of a full MUD.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Blinking Receiver}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
When a single-user employs the TH-IR scheme, the optimum detector
is a correlation receiver. The samples at the matched filter
output are summed and a decision in made thereupon. In a
multi-user scenario collisions typically introduce interference.

The blinking Receiver (BR) \cite{fishler-lowcomplexity} is a basic
multi-user detector. It considers only those information bits not
corrupted by collisions with other users.
%Its decision %The output of the BR
%is based only on its received pulses not perturbed by collisions
%of the user of
%interest where no collision occurred.
The BR can be described by using the collision designating vector
$w^T_{k}$ as follows
%
\begin{equation}\label{br-output}
    \hat{b_k} = sgn(w^T_{k}r_k),
\end{equation}
%
where $\hat{b_k}$ is the estimation for user $k$, and
$sgn(x)\equiv{x/\left|x\right|}$. The main advantages of the BR
receiver are its simplicity and ease of analysis.
%that it can be easily analyzed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{SMUD channel model}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
In the above system model each information symbol is repeated %transmitted
$N_f$ times. Each of these repeated symbols is transmitted in one
chip chosen randomly from $N_c$ available chips. The chip duration
is $T_c$. A sequence of $N_c$ chips constitutes a frame.
%
\begin{figure}[ht]
    \centering
    \includegraphics{eps/channel_model}
    \caption{System illustration}
    \label{fig:SystemModel}
\end{figure}
%
Figure~\ref{fig:SystemModel} depicts a toy example of transmitting one
information symbol in a 2-user system with the following parameters:
$N_f=3$ frames, $N_c=5$ chips per frame. The rectangles represent the slots
used by the users. In this example the collision designating vector associated
with user $1$ is $w_1 = [1,0,1]$.

%
In order to analyze this system we propose a simple
%the following
system model. It based on the fact that it suffices to consider a
%communication scheme with a
single frame consisting of $N_c$
chips. Each user transmits its information using a single,
randomly-chosen, chip position. (Note that by employing repetition
code of length $N_f$ one returns to the original system model.)
%
According to this model $r$ is the vector
$[r_1,r_2,\ldots,r_{N_c}]$, and $r_k=r_{c^k}$. Note that for each
frame, only one pulse position $c^k$ needs to be randomized.

We begin with a "hard-decision" channel model; the corresponding channel
output $Y$ is defined as
%will be defined by
%
\begin{equation}\label{hard_dec_model}
    Y = \left\{ \begin{array}{ll}
        sgn(r_k)    & \textrm{$w_k\ne{1}$} \\
        \epsilon    & \textrm{$w_k=1$}.
        \end{array} \right.
\end{equation}
%
A collision in this model will be treated as an \emph{erasure},
labelled by $\epsilon$.

Let $e$ denote the erasure (collision) probability %of an
per chip, and let $\mu$ be the probability of an error when no
collision occurs. Clearly,
%
\begin{equation}\label{hard_dec_peps}
    e = 1-(1-\frac{1}{N_c})^{K-1},
\end{equation}
\begin{equation}\label{hard_dec_pe}
    \mu = Q(\frac{A_k}{\sigma_n}),
\end{equation}
where
$Q(\beta)\equiv\int^{\infty}_{\beta}\frac{e^{-\alpha^2/2}}{\sqrt{2\pi}}d\alpha$.
%
Figure~\ref{fig:bee_cahnnel} depicts the corresponding channel
model

\begin{figure}[ht]
    \centering
    \includegraphics[width=180pt]{eps/bee_hard_channel}
    \caption{Binary erasure with errors (hard decision) channel}
    \label{fig:bee_cahnnel}
\end{figure}

The Shannon capacity associated with this channel is given by
% this
%channel model for which we can obtain the Shannon capacity:
% for this channel and now we
%can get its capacity :
%
\begin{equation}\label{hard_dec_capacity}
    C_{hard} = (1-h(\mu))(1-e),
\end{equation}
where $h(p)=-plog(p)-(1-p)log(1-p)$.

Next, we consider a "soft-decision" channel model; the corresponding channel
output $Y$~is~defined~as
%A channel model with soft output $Y$ can be described as
\begin{equation}\label{soft_dec_model_2}
    Y = \left\{ \begin{array}{ll}
        X+n         & \textrm{$w_k\ne{1}$} \\
        \epsilon    & \textrm{$w_k=1$},
        \end{array} \right.
\end{equation}
where $X$ is the channel (binary) input chosen from $\{1,-1\}$ and
$n$ is additive Gaussian noise. Figure~\ref{fig:bee_soft_cahnnel}
shows a schematic model for this channel.

\begin{figure}[ht]
    \centering
    \includegraphics[width=200pt]{eps/bee_soft_channel}
    \caption{Binary input - soft output with erasures}
    \label{fig:bee_soft_cahnnel}
\end{figure}

This channel is a BAWGN channel with erasures; its capacity is
given by
\begin{equation}\label{soft_dec_capacity}
    C_{soft} = (1-e)C_{BAWGN},
\end{equation}
where $C_{BAWGN}$ is the capacity of BAWGN channel:
\begin{equation}\label{bawgn_capacity}
\begin{split}
    C_{BAWGN} = &\frac{1}{2}\int_{-\infty}^{\infty}p(y|A)log_2\frac{p(y|A)}{p(y)}dy +\\
                          &\frac{1}{2}\int_{-\infty}^{\infty}p(y|-A)log_2\frac{p(y|-A)}{p(y)}dy.
\end{split}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{High SNR channel analysis}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%

Interestingly, %Note that
for a given number of chips $N_c$, each
user sees its own channel with a capacity %that is only
affected only by its own signal-to-noise ratio (SNR) and the
number of users - but not by the signal powers of other users.
%
Consequently, in the high-SNR regime % Lets assume that the SNR is high. In this
%case we get
$\mu\rightarrow0$, and both the hard-decision and the
soft-decision models behave as
%the channel model of both the decoders become
a binary erasure channel (BEC) whose capacity is given by
\begin{equation}\label{high_snr_capacity}
    C_{highsnr}= 1-e = (1-\frac{1}{N_c})^{K-1}.
\end{equation}
%

Using repetition coding over this channel, % model,
as assumed by the BR receiver, can never achieve zero error rate
unless the rate (bits/frame) goes to zero.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{SMUD simulation results}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%

We evaluate by simulation the performance of a multi-user system
employing the BR receiver. The BER performance of the system is
measured for several SNR values and for $N_c = 20$ chips per
frame. The SNR is given by $SNR=10log\frac{E_s}{N_0}$, where 
$E_s$  is the energy expanded per channel use. 
%The signal power is the energy of one pulse.
%The SNR is taken per pulse (disregarding code rate) to be able
%to compare with capacity
%Repetition code is used since the BR receiver is intended for such
%codes.
We shall be considering different data rates, i.e. different
values of $N_f$, where $Rate = 1/N_f$ is the (average per-user)
number of bits per frame.
% it is obvious from here that the code is repetition.
%
We begin with a small number of users $K=3$. In this case, the
erasure probability (\ref{hard_dec_peps}) is $e_{K=3} = 0.0975$,
and the maximum achievable capacity in the interference-limited
regime is $C_{high-snr, K=3} = 0.9025$.
%(when $SNR\rightarrow\infty$, i.e.  ).
% note : was before - maximum capacity
%
%Figure~\ref{fig:blinking_reciver_sim_3user} presents the
%simulation results for this case.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]
            {python_graphs/blinking_reciver_sim_3user/blinking_reciver_sim_3user}
    \caption{blinking receiver, $K$=3 users}
    \label{fig:blinking_reciver_sim_3user}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]
            {python_graphs/blinking_reciver_sim_11user/blinking_reciver_sim_11user}
    \caption{blinking receiver, $K$=11 users}
    \label{fig:blinking_reciver_sim_11user}
\end{figure}
%
Figure~\ref{fig:blinking_reciver_sim_3user} presents the
simulation results for this case. Ha {\it et al.}
\cite{ldpc_biawgn_erasures} analyzed and optimized the performance
of LDPC codes for use over the BAWGN channel. Although the actual
channel assumed by Ha is different from the one presented herein,
the system model is similar, and hence we include in the figure
some (optimized) LDPC results for comparison.
%
%Next, we added two point of actual LDPC coded system.
%
For $SNR=4dB$ and system BER of $10^{-4}$, one can obtain rate of
$0.8[\frac{bit}{frame}]$ by using a certain optimized LDPC code.
Also, for rate of $0.5[\frac{bit}{frame}]$, one can obtain BER
of $10^{-5}$ with $SNR=-1.25dB$ by using LDPC coding. One can not
come close to this rate/BER/SNR with the BR receiver employing
repetition coding.
%
%(Note that the results corresponding to LDPC coding are associated
%with two different LDPC codes. Each of these was optimized
%according to specific system parameters.)
%
%
%
%% removed beacuse incorrect 
%%Finally, the dashed line represents the theoretical capacity
%%achievable with $SNR=0.2dB$. This SNR value has been chosen in
%%order to show the theoretical performance in a rather noisy
%%system, (but also since this point corresponds to the analysis in
%%\cite{ldpc_biawgn_erasures}.)


Next, we consider a system with a large number of users, $K=11$.
In this case the erasure probability is $e_{K=11} = 0.4$, and the
maximum achievable capacity in the interference-limited regime is
 $C_{high-snr, K=11} = 0.6$. The results are presented in
Figure~\ref{fig:blinking_reciver_sim_11user}.
%Again, the
%theoretical capacity is marked as a dotted line and the point
%represents result taken from \cite{ldpc_biawgn_erasures}.
The behavior and conclusions are similar to the previous scenario.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Conclusion}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%In this chapter we presented the SMUD. We suggested a more general system
%model, and by using this model we calculated the theoretical
%capacity of the system. The original decoding scheme performance
%is not close to capacity and by using a coded scheme we can
%approach capacity.
%
Motivated by the huge gap from the theoretical bounds, in the next section we introduce coding into the system and present a full multi-user detector.
%Motivated by the performance of LDPC results we will introduce a coded scheme aimed at
%improving performance.

